Value-based Fast and Slow AI Nudging

Nudging is a behavioral strategy aimed at influencing people's thoughts and actions. Nudging techniques can be found in many situations in our daily lives, and these nudging techniques can targeted at human fast and unconscious thinking, e.g., by using images to generate fear or the more careful and effortful slow thinking, e.g., by releasing information that makes us reflect on our choices. In this paper, we propose and discuss a value-based AI-human collaborative framework where AI systems nudge humans by proposing decision recommendations. Three different nudging modalities, based on when recommendations are presented to the human, are intended to stimulate human fast thinking, slow thinking, or meta-cognition. Values that are relevant to a specific decision scenario are used to decide when and how to use each of these nudging modalities. Examples of values are decision quality, speed, human upskilling and learning, human agency, and privacy. Several values can be present at the same time, and their priorities can vary over time. The framework treats values as parameters to be instantiated in a specific decision environment.

==> after_end.tex <==



%ANDREA: queste references vanno aggiunte al .bib
%(ma il .bib nancora on funziona)

%Andrea, ho aggiunto anche queste:

%-- Ackerman2017
%Ackerman R., Thompson V. A. (2017) Meta-Reasoning: Monitoring and Control of Thinking and Reasoning, Trends in Cognitive Sciences, 21(8), 607-617

%--Carruthers
%Carruthers, P. (2021) Explicit nonconceptual metacognition. Philosophical Studies 178(2337–2356)

%--Kim2019
%Kim, D., Park, G.Y., O′Doherty, J.P. et al. (2019) Task complexity interacts with state-space uncertainty in the arbitration between model-based and model-free learning. Nat Commun 10(5738) https://doi.org/10.1038/s41467-019-13632-1

%-- Proust2004
%Proust, J. (2014). The philosophy of metacognition. Oxford: Oxford University Press.

%-- Shenhav2013
%Shenhav, A., Botvinick, M. M., & Cohen, J. D. (2013). The expected value of control: an integrative theory of anterior cingulate cortex function. Neuron, 79(2), 217–240. https://doi.org/10.1016/j.neuron.2013.07.007

%-- Thompson2011
%Thompson V., Turner J.P., Pennycook G. (2011) Intuition, reason, and metacognition, Cognitive Psychology, 63(3), 107-140



%-- Cox2005
%Cox, M. T. (2005) Metacognition in computation: A
%selected research review. Artificial intelligence, 169(2):
%104–141

%-- CoxRaja2011
%Cox M. T. and A. Raja, Metareasoning: Thinking about Thinking. The MIT Press, 2011.

%-- Fagin2003
%Fagin, R.; Moses, Y.; Halpern, J. Y.; and Vardi, M. Y. (2003). Reasoning about knowledge. MIT press

%-- Flavell1979
%Flavell, J. (1979). Metacognition and cognitive monitoring: A new area of cognitive-developmental inquiry. American Psychologist, 34, 906–911.

%-- marcus2020next
%Marcus, G. (2020). The next decade in AI: Four steps towards robust artificial intelligence. arXiv preprint arXiv:2002.06177 .

%--kahneman2011thinking
%Kahneman, D. (2011). Thinking, Fast and Slow. Macmillan.


%-- Kralik2018
%Kralik et al.,(2018) Metacognition for a common model of cognition. Procedia Computer Science, 145 

%-- NN1990
%Nelson, T., & Narens, L. (1990). Metamemory: A theoretical framework and new findings. In G. Bower (Ed.), The psychology of learning and information. Cambridge: Academic Press.

%-- Posner2020
%Posner, H., (2020) Robots thinking fast and slow: on dual process theory and metacognition in embodied AI. Robotics Retrospectives.

%-- RossiThinking (c'e' gia' nel .bib, e adesso e' chiamato aaai2021-blue)

%-- RossiLoreggia2019 (c'e' gia, chiamato rossi2019preferences)
%Rossi, F. and Loreggia, A. (2019). Preferences and ethical priorities: Thinking fast and slow in AI. In Proceedings of the 18th International Joint Conference on Autonomous Agents and Multi-Agent Systems (AAMAS), 3–4.





\section{Explaining design-choices. }
We design a metacognitive module with S1 and S2 modality because we expect it to provide more flexibility and optimality than a single-modality metacognition. Because S1MC takes into account less data and needs to compute less knowledge than S2MC for its decision-process, S1MC is a shallower but also a less costly agent than S2MC. This is the optimal metacognitive agent to use when the S1solver has experience with the task and may have already successfully solved that same task in the past. In contrast, when the stakes are high and the S1solver provides a solution with a low degree of confidence, it is optional to engage a more reflective form of metacognition. 
In line with our general designed choices about S1 and S2 agents, S1MC starts automatically when a task comes in and a solution is provided by the S1solver. That eliminates the burden of explaining what initially activates metacognition (and potentially facing  a regress problem). In contrast, because S2MC is more resource-hungry than S1MC, it can only be activated by S1MC as to avoid any unnecessary waist of resources.  



\section{Various material}

MC design choices:

\begin{itemize}
    \item 
Only one MC module (not distributed), though the MC can subcontract parts of the evaluation to more specialized metacognitive agents (e.g. epistemic, moral): 
Justification: we assume that solvers do not have access to the necessary info to make metacognitive decisions (e.g., past performances in similar tasks). Also, solvers can’t decide what tasks to prioritize.  

\item Sequential S1 and S2 assessment modalities in the MC module: 
\begin{itemize}
    \item Justification for having a S1 MC: the MC needs to be flexible to avoid consuming unnecessary time and resources that should be allocated otherwise. 
    \item A S1 MC agent allows for this flexibility and so should be part of our design and the first kind of assessment to be triggered.
\end{itemize}
\item S1MC is not simply a rough version of S2MC: S2 MC decides between S1 vs S2 solver (or opt out). S1MC has the job to decide between adopting S1 solution or engaging S2 MC based on value of success and past experience 
\item In terms of efficiency, it does not make sense to engage in a cost-benefit analysis of S1 vs S2 solvers [i.e. the job of S2MC] if 
the system has already successfully solved the task
the value of success is so low to the point that an imperfect solution is acceptable   
\item So UNLESS the value is high, our design choice is to check past solutions / success before any (rational) cost -benefit analysis 
\item Justification for why S1 MC starts automatically: we want to avoid the need to have to choose when to engage the MC module. 
%\end{itemize}

\item The solver agents and the MC module communicate about solutions, failed attempts, estimated time to completion, etc
\begin{itemize}
    \item 
Justification: after reaching a decision about arbitration, the S1 MC assessment continuously monitors the inputs (time, resources, value of success), the inner workings and results coming from the solver agent. The reason is that the S1 MC might need to adjust its decision in course of action (e.g., switch to S2 to S1, opt out)
\end{itemize}
\item 
No direct route from S1 MC to the S2 solver agent: S1 MC could engage S2 MC or accept the solution of an S1 Solver
\begin{itemize}
    \item Justification: S1 MC is too shallow to be able to assess whether or not to engage a potentially time-consuming S2 solver. In order to engage S2 solvers a more deliberate and careful S2 MC agent is needed.
\end{itemize}
\end{itemize}
%\end{itemize}

\section{System 1 agents}

   \begin{itemize}
        \item relying on past experience
        \item self-activating
        \item confidence level on provided solution
        \item 2 kinds: model builders and model users
        \item O(1) computational complexity (for model users)
        \end{itemize}
        
\begin{itemize}
    \item S1 agents/ automatically activated agents  
\item Model builder: Model-builder based on data from past experience / raw data; and updater based on new data/ decisions 
\begin{itemize}
    \item 
They activate when new data come in from the outside 
\end{itemize}
\item S1 solver-model user:
\begin{itemize}
    \item 
O(1) computational complexity 
\item Looks at past experience in the model of the self
\item Activates only automatically
\item An S1 solver activates itself only if it has the abilities and system’s knowledge for a detected task 
\item Activates as soon as a task comes in
\item If task is too complex S1 does not provide any answer 
\end{itemize}
\end{itemize}

Alternative solutions and amendments (they won’t be adopted now but will be considered when the above design has been tested): 



     
\section{System 2 agents}

    \begin{itemize}
    \item reasoning on the current problem
    \item activated by meta-cognitive module
       \end{itemize}
          
           
           S2 agents / consciously  activated agents  

Always activated by a MC module 
Slow thinking: 
Uses rational methods, cost-benefit analysis
Not experience based  


\section{Meta-cognition}

    \begin{itemize}
        \item functions (arbitration, self-control, ...)
        \item system 1 and system 2 components
        \item assessment factors and computation
    \end{itemize}
        
 Meta-cognitive module’s functionalities:

\begin{itemize}
    \item 
Monitoring and integrating data coming from:
\begin{itemize}
    \item 
Model of the Self  
\item Model of Others
\item Model of the World 
\item External world 
\end{itemize}
\item Arbitration between S1/S2 (or opting out) for one task at the time (for now) 
%\end{itemize}

\item S1 MC: 
\begin{itemize}
    \item 
First: evaluation of value of success
\item If value is low, evaluation of S1 solver’s solution (if any):
\item Accepts S1 solution if reliable (high value of confidence), or if not enough resources to engage S2MC  
\item Engages S2MC if value of success is high or S1 solver’s solution is not reliable  or not present
\end{itemize}
\item S2 MC:
\begin{itemize}
    \item 
Cost-benefit analysis of using S1/S2 solvers: maximizing expected value of control 
\item Careful evaluation of S1 solutions
\item Cost-benefit of using S2 solver
\item When opting out?
\item Reflection and self-improvement: 
Assess the quality of solvers’ performances (for each task: time, success, energy needed, ...)
Asses failure and cause of failure in solvers [see Aqua] 
Inform/ write about solvers’ performances (based on self-imposed constraints - time, success, energy needed, ...) on the model of the self  
Goals generation (e.g. adjusting goals based on available resources)
Invocation, aborting solvers as needed  
\end{itemize}

\begin{itemize}
    \item S1 should be much simpler, only looking at resource constraints 
\item S1 is not needed, MC should only be a S2 modality 
\item S2 is not needed, MC should only be a S1 modality
\item MC is distributed. The solvers also have some metacognition capabilities.
\item Arbitration between S1 and S2 when multiple tasks are given in a batch (synchronous) + in a stream (asynchronous)
\item Learn new skills / hone existing skills, as a meta-level decision for self-development of the population of agents
\end{itemize}
\end{itemize}

\section{Use cases to show specific instances of the framework}
%: sequential decision making in a constrained grid environment}

\begin{itemize}
    \item epistemic planning: optimizing planner selection 
    \item human reasoning (our workstream + Aanya's work): modelling human reasoning in sequential decision environments
    \item moral judgement: supporting humans in moral decisions by providing a system 2 rationalization in high-stake moral judgements
\end{itemize}


%\section{References (to be moved to bibliography}

%References:

%Metacognition: 

%CoxRaja2011
%M. T. Cox and A. Raja, Metareasoning: Thinking about Thinking. The MIT Press, 2011.

 
%S. Russell and E. Wefald, “Principles of metareasoning,” Artificial intelligence, vol. 49, no. 1-3, pp. 361–395, 1991. 

%S. Milli, F. Lieder, and T. L. Griffiths, “When does bounded-optimal metareasoning favor few cognitive systems?” in Thirty-First AAAI Conference on Artificial Intelligence, 2017

%H. Posner, “Robots thinking fast and slow: on dual process theory and metacognition in embodied ai.” Robotics Retrospectives, 2020

%Kralik et al. (2018), "Metacognition for a common model of cognition", Procedia Computer Science, 145 


%S1-S2 design: 

%G. Goel, N. Chen, and A. Wierman, “Thinking fast and slow: Optimization decomposition across timescales,” SIGMETRICS Perform. Eval. Rev., vol. 45, no. 2, pp. 27–29, Oct. 2017. [Online]. Available: http://doi.acm.org/10.1145/3152042.3152052 
%J. Xie, Z. Zheng, X. Fang, S.-C. Zhu, and Y. N. Wu, “Multimodal conditional learning with fast thinking policy-like model and slow thinking planner-like model,” arXiv preprint arXiv:1902.02812, 2019. 
%S. Mittal, A. Joshi, and T. W. Finin, “Thinking, fast and slow: Combining vector spaces and knowledge graphs,” ArXiv, vol. abs/1708.03310, 2017. 
%T. Anthony, Z. Tian, and D. Barber, “Thinking fast and slow with deep learning and tree search,” in Proceedings of the 31st International Conference on Neural Information Processing Systems, ser. NIPS’17. USA: Curran Associates Inc., 2017, pp. 5366–5376. [Online]. Available: http://dl.acm.org/citation.cfm?id=3295222.3295288
%D. Chen, Y. Bai, W. Zhao, S. Ament, J. M. Gregoire, and C. P. Gomes, “Deep reasoning networks: Thinking fast and slow,” ArXiv, vol. abs/1906.00855, 2019. 
%U. Kannengiesser, J. S. Gero, Y. Eriksson, and K. Paetzold, “Empirical evidence for Kahneman's system 1 and system 2 thinking in design,” Human Behavior in Design, pp. 89–100, 2019.
%A. Augello, I. Infantino, A. Lieto, U. Maniscalco, G. Pilato, and F. Vella, “Towards a dual process approach to computational explanation in human-robot social interaction,” in CAID@ IJCAI, 2017
%D. Fridovich-Keil, S. L. Herbert, J. F. Fisac, S. Deglurkar, and C. J. Tomlin, “Planning, fast and slow: A framework for adaptive real-time safe trajectory planning,” in 2018 IEEE International Conference on Robotics and Automation, ICRA 2018, Brisbane, Australia, May 21-25, 2018, 2018, pp. 387–394. [Online]. Available: https://doi.org/10.1109/ICRA.2018.8460863 

%G. Booch, F. Fabiano, L. Horesh, K. Kate, J. Lenchner, N. Linck, A. Loreggia, K. Murugesan, N. Mattei, F. Rossi, and B. Srivastava, “Thinking fast and slow in ai,” 2021


%Different types of thinking:

%F. D. Lellis, F. Auletta, G. Russo, P. D. Lellis, and M. di Bernardo, “Control-tutored reinforcement learning,” 2019. 
%M. Rathi, P. Ferraro, and G. Russo, “Driving reinforcement learning with models,” 2020

%\input{content-files/sec-motiv-evaluation}

%\input{content-files/sec-usecases}
%\input{content-files/sec-background}

%\appendix
%\input{content-files/sec-old-introduction}


% --------------------
%\subsection*{Acknowledgments}

%\bibliographystyle{abbrv}
%\bibliography{bibs/abb,bibs/thinking_aaai21,bibs/s1s2}

\bibliographystyle{abbrv}
\bibliography{biblio}


\end{document}

%{
%\small
%\bibliographystyle{aaai21.bst}
%\bibliography{abb,thinking_aaai21} 
%}

%\end{document}

% --------------------


==> authors_list.tex <==
Marianna B. Ganapini ( Union College ) < bergamam@union.edu> 
Arie Glazier ( Tulane University ) < adglazier@gmail.com> 
Murray Campbell ( IBM Research ) < mcam@us.ibm.com> 
Francesco Fabiano ( University of Udine ) < francesco.fabiano@uniud.it> 
Lior Horesh ( IBM Research ) < lhoresh@us.ibm.com> 
Jon Lenchner ( IBM Research, USA ) < lenchner@us.ibm.com> 
Andrea Loreggia ( University of Brescia ) < andrea.loreggia@gmail.com> 
Nicholas Mattei ( Tulane University ) < nsmattei@tulane.edu> 
Taher Rahgooy ( University of West Florida ) < trahgooy@students.uwf.edu> 
Francesca Rossi ( IBM Research ) < Francesca.Rossi2@ibm.com> 
Biplav Srivastava ( Univ. of South Carolina ) < biplav.s@sc.edu> 
Brent Venable ( Institute for Human and Machine Cognition ) < bvenable@ihmc.org> 
